Squish: Near-Optimal Compression for Archival of Relational Datasets

Relational datasets are being generated at an alarmingly rapid rate across organizations and industries. Compressing these datasets could significantly reduce storage and archival costs. Traditional compression algorithms, e.g., gzip, are suboptimal for compressing relational datasets since they ignore the table structure and relationships between attributes. We study compression algorithms that leverage the relational structure to compress datasets to a much greater extent. We develop Squish, a system that uses a combination of Bayesian Networks and Arithmetic Coding to capture multiple kinds of dependencies among attributes and achieve near-entropy compression rate. Squish also supports user-defined attributes: users can instantiate new data types by simply implementing five functions for a new class interface. We prove the asymptotic optimality of our compression algorithm and conduct experiments to show the effectiveness of our system: Squish achieves a reduction of over 50\% in storage size relative to systems developed in prior work on a variety of real datasets.

==> analysis.tex <==
\section{Theoretical Analysis}

In this section, we prove that our compression algorithm achieves near optimal compression rate. We bound the expected length of the code string of each tuple in terms of the entropy of the tuple. 

\begin{theorem}
Suppose that all tuples in our database are independently sampled from population distribution $p$. Then for another random tuple $t$ sampled from $p$, the expected length of the encoded string of $t$ is bounded by:
$$ \mathbb{E}_p[\mathbf{len}(\textit{code}(t))] \leq H_p(t) + D(p||M) + 2 $$
where $D(p||M)$ is the KL divergence of population distribution $p$ and our modeled distribution $M$. $H_p(t)$ is the entropy of distribution $p$.
\end{theorem}

Note that if $p$ can be expressed using probabilisitic graphical model, then for some model $M$ the above upper bound is nearly tight (since for any tuple $t$, the minimum number of bits to encode $t$ is the entropy of $t$). In probabilistic graphical model literature, it is well known that given sufficiently large training dataset, optimizing under the minimal description length principle leads to the exact underlying model. Thus our compression algorithm will achieve near entropy compression rate if training data is sufficiently large.

